Understanding the Complexity of Detecting Political Ads

Online political advertising has grown significantly over the last few years. To monitor online sponsored political discourse, companies such as Facebook, Google, and Twitter have created public Ad Libraries collecting the political ads that run on their platforms. Currently, both policymakers and platforms are debating further restrictions on political advertising to deter misuses. This paper investigates whether we can reliably distinguish political ads from non-political ads. We take an empirical approach to analyze what kind of ads are deemed political by ordinary people and what kind of ads lead to disagreement. Our results show a significant disagreement between what ad platforms, ordinary people, and advertisers consider political and suggest that this disagreement mainly comes from diverging opinions on which ads address social issues. Overall our results imply that it is important to consider social issue ads as political, but they also complicate political advertising regulations.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> background.tex <==
%!TEX root = paper.tex

\section{Background}

We review next the definitions and restrictions for political advertising across various ad platforms. 

\vspace{1mm}
\noindent \textbf{Facebook} defines political ads as~\cite{facebook-political-ads}: \textit{
Made by, on behalf of, or about a candidate for public office, a political figure, a political party or advocates for the outcome of an election to public office; or
About any election, referendum or ballot initiative, including "go out and vote" or election campaigns; or
About social issues in any place where the ad is being placed; or
Regulated as political advertising.}

Everyone with a Facebook account can be an advertiser if they provide a payment method. However, to be able to send political ads advertisers need to verify their account by providing proof of their identity card~\cite{facebook_adv}. Advertisers can only send political ads in the country they reside and need to provide proof of residence. Advertisers need to self-label if their ads are political and need to provide a 
disclaimer about who paid for the ad. This paid\_for\_by disclaimer appears on the top of the ad after the advertiser's name.  Finally, political ads will be added to the Facebook Ad Library~\cite{facebook-ad-library}.


\vspace{1mm}
\noindent \textbf{Google} defines political ads as: \textit{ads about political organizations, political parties, political issue advocacy or fundraising, and individual candidates and politicians}~\cite{google-political-ads}. 
There are no restrictions imposed by the platform on political ads, but the platform expects all political ads to comply with local legal requirements. 

Google considers election ads as a separate category. The definition of election ads depends on the country  but overall it refers to only ads from or about candidates and political parties in the election.  Only verified advertisers are able to run election ads.  Election ads can only be targeted to geographic location (except radius around a location), age, gender and contextual targeting options such as ad placements, topics, keywords against sites, apps, pages and videos. 

\vspace{1mm}
\noindent \textbf{Twitter} defines political ads as \textit{ads with political content: that references a candidate, political party, elected or appointed government official, election, referendum, ballot measure, legislation, regulation, directive, or judicial outcome; as well as ads of any type by candidates, political parties, or elected or appointed government officials}~\cite{twitter-political-ads}. 
Twitter bans all political ads.  
 
\vspace{1mm}
\noindent \textbf{TikTok}
defines political ads as \textit{ads that promote or oppose a candidate, current leader, political party or group, or issue at the federal, state, or local level — including election-related ads, advocacy ads, or issue ads}~\cite{TikTok}. 
TikTok bans all political ads.  




==> comparison.tex <==
\section{Analyzing ad labeling}
\label{sec:label comaprision}
This section looks at the ads volunteers consider as political and then analyzes the differences between these ads and the ads labeled as political by advertisers. 

\input{labels_volunteers}

\input{labels_advertisers}

%\input{labels_comparison}



==> extra.tex <==

\section{Extra}
 
\paragraph{Analysis of ad messages using topic models}

To understand differences and similarities in the ad messages between different groups of ads we use topic models to analyze them.
To extract topics we used(LDA) with Bag of Words using the python package \update{XX}.  To extract topics we used all \update{XX} ads in the ProPublica dataset. We varied the number of topics to extract from 30 to 65.  In our case with 55 topics we achieved the most interpretable result (the topics were unique, interpretable and diverse). You can see in Table~\ref{XX} in Appendix~\ref{XX} the 10 most important words for each topic with the number of ads assigned to the topic. 

For each group of ads we select the four most popular ad topics. Table \ref{tab:lda} and Figure~\ref{fig:LDA} present the breakdown in topics for different ad groups. 
\subsection{Political speech: a legal perspective} 

\oana{here we need to discuss laws that regulate political speech. Political speech is has its own legal status and often has additional protection. EU Member states  have different laws and different provisions for political speech}

\oana{check this doc for definitions and legal perspectives on political speech/advertising: \url{https://www.stiftung-nv.de/sites/default/files/rules_for_fair_digital_campaigning.pdf}}

\oana{also check the references in this doc: https://epd.eu/wp-content/uploads/2020/09/joint-call-for-universal-ads-transparency.pdf }

\oana{we need to talk about EU Member State laws on political advertising}. \oana{Check this: 
ERGA?s noted that the definitions of political ads and issue-based ads adopted by the platforms are inconsistent with the requirements set out in EU Member State laws, where they
exist, although they do not exist in many countries. See ERGA, Report of the activities carried out to assist the European Commission in the intermediate monitoring of the Code of
practice on disinformation, June 2019, p. 15, available here.
\url{https://erga-online.eu/wp-content/uploads/2019/06/ERGA-2019-06_Report-intermediate-monitoring-Code-of-Practice-on-disinformation.pdf}}

Political speech online differs in nature and legislation from other advertising. As inherently contested speech, political speech has its own legal status with additional protection, and is in many countries subject to specific laws and restrictions. The potential impact of online political ads is also far greater and more harmful. Where you might buy the wrong hair drier because of a highly targeted commercial ad, you might end up voting for a party whose programme contradicts your values and interests because of highly targeted political ads. It is therefore essential to look at political advertising and properly regulate this space that is so essential to our democratic processes.




\section{LDA}

\textbf{Strong political ads}, \pa and \opa have 2 common topics out of 4 most popular. \textbf{Marginally political ads} have one topic in common with \pa and have one topic in common with \opa. Only \spa and \pnpa do not have any intersection between topics. 
All three topics from \spa are highly related to the political figures or the election process. On the contrary, themes from \npa are about different social issues such as human welfare and other themes are related to the product ads (like topics 5 and 6). Finally, the topics from \pa and \opa are more diverse. They have themes that are about political persons or political parties. Nevertheless, some topics are about people activism and human rights. 


\begin{table}[]
    \centering
    \small{
    \begin{tabular}{|p{0.01\textwidth}|p{0.45\textwidth}|}
    \hline
       & Topic \\
      \hline
        1 & donate gift today help match impact time double dollar year\\
        \hline
        2& health care access abort right afford protect fight reproduction people\\
        \hline
        3&democrat mcconnel mitch senate defeat republican seat need midnight poll\\
        \hline
        4 & help need provide crisis family children water emergency food world\\
        \hline
        5& good time cook kind penzey value free thank email come\\
        \hline
        6& free american support thank sticker card member miss limit sign\\
        \hline
        7&trump president donald administrator fight stand stop protect hold need\\
        \hline
        8 &vote elect voter november candid ballot right poll like primary\\
        \hline
        9 & campaign donate help chip need grassroots goal today raise contribution\\
        \hline
    \end{tabular}
    }
    \caption{The most popular topics}
    \label{tab:lda}
\end{table}


\begin{figure}
    \centering
    \includegraphics[scale = 0.38]{plots/lda-2.pdf}
    \caption{The most popular ad topics (according to LDA) across different groups of ads.}
    \label{fig:LDA}
\end{figure}


\subsection{lables from advetisers}
\update{2\% of \spa and 13\% of \pa with disclaimer are labeled as non-political by workers. One reason for the difference is that volunteers can be influenced the paid\_for\_by label (workers did not see the paid\_for\_by label). This does not seem to be the case as the \vera{median fraction in all cases is 0.75(volunteers+label, volunteers - label, worker +label, workers - label)}. A second reason, as discussed in Section~\ref{XX}, is that workers might not have the necessary background knowledge identify political figures. We indeed see such anecdotal cases in the data.}  \oana{we need to have a more clear picture of the 13\% and 2\% is we want to discuss this. @vera}
\oana{not yet said anything about \pnpa with and without label. while volunteers do not consider these ads as political, workers consider 30-40\% of them as political. Is the definition that helped?}

\subsection{Classifiers}

\begin{table}[]
    \centering
    \begin{tabular}{||p{0.25\textwidth}|p{0.2\textwidth}||}
    \hline \hline
         & \opa \\
         \hline
       \spa, \pa, \pnpa  & 0.69\\
       \hline
       \spa, \pa & 0.63\\
       \hline
       \spa & 0.4\\
       \hline
       \pnpa & 0.1\\
       \hline
    \end{tabular}
    \caption{Intersection between \opa and other groups of ads}
    \label{tab:int opa and others}
\end{table}


\subsection{Copy-paste commetns}


\oana{we want to understand what they label as political but we also want to understand how good of a source they are }



\subsection{Discussion}

\paragraph{Which definition/instrumentation is better?}

\update{the goal of task design is to reduce confusion/increase agreement while keeping the diversity. one way to reduce confusion is to only consider ads from donnald trump }


Each group of ads is interesting in its own way: \spa are ads where everyone agrees that are political, hence, a-priori is reasonable to assume that they are easier to agree irrespective of who is labeling the ads (i.e., advertisers, volunteers or workers); \pa are ads where a majority of people would agree that they are political, hence, they are the ads that can help to refine and clear the definition of what is a political ad by understanding what are the reasons why some of the users \textit{do not} labeled the ads as political; and \pnpa are ads where there are some people considering the ads as political but not the majority. This group of ads might be a valuable source of diversity in political ads where we could find ads about local candidates, and new social issues that arise in particular groups of people that are not largely recognized.  

The majority of \spa are about the election process or well-known political persons (e.g., 2 out of 4 ads contain the name Donald Trump). The \pa are still strongly related to government and political actors, but they are more focused on human rights activism. Finally, \pnpa mostly focused on charity and social issues such as environmental politics and health.


\textbf{How political advertising is regulated at national levels --Oana}
While most countries have very detailed regulations on the transparency of political finance and limitations on political campaigning, few European countries have adapted these rules to the digital age. Many European countries? electoral regulations include silence periods, dedicated ad space on broadcasters, restrictions on the design and content of political ads, and spending caps, but these measures are rarely adapted to the new campaigning reality online. 




\begin{table*}
\footnotesize{
 \begin{tabular}{|p{0.15\textwidth}|p{0.8\textwidth}|}
 \hline
 Advertiser&Text \\  
 \hline
  \multicolumn{2}{c}{ \Pnpa \textbf{without 'paid\_for\_by' label}}\\
 \hline
This American Life &Republican Senator Jeff Flake is trying hard to get an immigration bill passed, working with a party he feels estranged from and a president who seems to hate his guts.\\
    \hline
  Knoxville News Sentinel & Check out what will be on the ballot for each district in the upcoming Knox County primary on March 3rd.\\ 
    \hline
    Institute for Southern Studies & When the courts keep striking down your laws as unconstitutional, what can you do? Take over the courts.\\
        \hline
    John Chiang&As Governor, John will fight against Trump's policies that will hurt California.\\ 

 \hline
  \multicolumn{2}{c}{ \Pnpa \textbf{with 'paid\_for\_by' label}}\\
 \hline
Melinda Gates &In the summer of 2017, a wave of stories forced the venture capital industry to start reckoning with its culture of sexual misconduct. I shared my perspective on what’s changed since then—and asked leaders in VC where we go from here.\\
    \hline
  The Intercept & This week on Intercepted, famed dissident Noam Chomsky breaks down the Trump presidency and explains why a life of resisting and fighting is worth it, and Hip Hop artist Bobby Sessions talks about police killings and this political moment.\\ 
    \hline
    Imprimis, a Publication of Hillsdale College & After Communism came identity politics.\\
        \hline
    The Arc of the United States&This \#GivingTuesday help us raise funds to protect the rights of people with intellectual and developmental disabilities!.\\ 
    \hline
    Solar Rebate & ATTENTION  OREGON HOMEOWNERS: There is a new policy that your power provider doesn't want you to know about. The Gov. Kate Brown will release \$100 million solar incentives for OR home solar expansion. If you are lucky enough to live in an active zip code, you can get paid to go solar. Check it out and see if you qualify!\\
    \hline
    DSA For The Many&DSA For the Many is raising money for four socialists who are running to shake-up the New York State legislature. We need to raise \$50,000 by May 18th so we can help them reach as many voters as possible.\\
    \hline
    Truthout&By making the legacy of pain in the United States inescapable, we can then lead ourselves into a legacy of remembrance, consideration and reparation.\\
    \hline
    The Christian Science Monitor&It could have long-term consequences.\\
    \hline
    Blue Wave 2018&Due to overwhelming demand, President Obama's famous "Democratic Donkey Polo" is now available for purchase...\\
 
 \hline
  \multicolumn{2}{c}{ \Pa \textbf{with 'paid\_for\_by' label}}\\
 \hline
PragerU&Before starting down the path to college, some common sense reflection is more necessary than ever. Charlie Kirk of Turning Point USA provides some much needed tutoring.\\
    \hline
  Consumers for Quality Care&New survey finds California voters want more clarity, information lower costs in health care.\\
    \hline
\end{tabular}
}
\caption{Examples of \pnpa and \pa with and without 'paid\_for\_by' disclaimer.}
\label{tab:exmp_lpa}



TO DO:
\begin{itemize}
    \item we should do a test on prolific to ask about issue in this ad group as well
    \item  compare ads from volunteers and advertisers only after 24/05/2018
\end{itemize}


\end{table*}

==> labels_advertisers.tex <==
%!TEX root = paper.tex

\subsection{Analyzing ad labels from advertisers}
\label{sec:labels advertiser}


In this section we analyze ads labeled as political by advertisers and compare them with ads labeled as political by volunteers. Table~\ref{tab:overlap} presents the overlap between ads labeled as political by volunteers the \opa (ads labeled as political by advertisers). The table shows that 96\% of \spa,  93\% of \pa and 74\% of \pnpa were also declared as political by advertisers. 

This is a bit surprising as we expected larger overlaps for \spa than \pnpa (i.e., what is considered as highly political by volunteers will also be considered as highly political by advertisers). Even more confusing, there are 1.3k ads where volunteers have consensus that they are non-political, but advertisers label them as political. Hence, \textit{there is a significant discrepancy between what advertisers labeled as political and what volunteers labeled as political.} 

There are three particular groups of ads that we give special attention: \spa and \pa without paid\_for\_by disclaimer because they corresponding to advertisers that should have labeled their ads as political but did not; \pnpa with paid\_for\_by disclaimer because they corresponding to ads that volunteers underreport, and \npa  that have the paid\_for\_by disclaimer because they correspond to advertisers that seem to wrongly label their ads as political. 

Table~\ref{tab:overlap} shows that 4\% of  \spa and 7\% of \pa did not have the paid\_for\_by disclaimer. 

We investigate whether the Facebook pages of the corresponding advertisers still exists. 66\% of ads that are in \spa and 62\% in \pa but not in \opa come from advertisers that no longer exist on Facebook. For comparison, this fraction is only 8\% if we look at ads in the \spa that are also in the \opa group. Hence, \textit{we see that the majority of the ads that were not declared as political by advertisers in the \spa and \pa group come from advertisers that no longer have a Facebook page}. We have no way to know whether Facebook removed these pages in an effort to remove malicious players that do not comply with their policies or if the advertisers themselves removed their pages to remove a proof of existence. {\color{red}(No longer relevant: now we have smaller amount of NA categories in the not official data. As percentage, it is the same as official data)} \textit{As observed by \citet{silva2020facebook} as well, there are advertisers that do not respect the platform policies on political ad declaration, which can explain in part discrepancies between labels from advertisers and volunteers.} {\color{red} No longer relevant }

\begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.4]{plots/plot_merg_with_np_data_new.pdf}  
    \vspace{-4mm}
    \caption{NEW VERSION: Breakdown of advertisers categories for different groups of ads  for ads with and without paid\_for\_by disclaimer.}
    \label{fig:all_categories_disclaimer_new}
   \vspace{-2mm}
\end{figure*}

\
\paragraph{Analyzing advertisers categories}
Figure~\ref{fig:all_categories_disclaimer_new} presents the breakdown of the categories of the corresponding advertisers for \spa, \pa, and \pnpa with and without disclaimer separately.  On the positive site we see that \opa come from a wide range of advertisers such as political actors and advocacy groups, but also NGOs, news medias and businesses. On the negative site, we see that a significant fraction of advertisers in \spa, and \pa without disclaimer are political actors and advocacy groups (29\% and 35\% respectively) which we would have expected to label their ads appropriately.

If we look at advertisers in \pnpa with disclaimer (ads that are considered political by advertisers, but that are confusing volunteers), \textit{we observer that volunteers seem to underreport ads from news media, non-governmental organizations (NGOs), and business. Hence, this emphasizes again the need for clear policies on the weight of advertisers' categories in ad labeling.} 

Finally, Figure~\ref{fig:all_categories_disclaimer} shows that many \npa with disclaimer come from NGOs, news media, businesses, charities and {\color{red} entertainment}. There are various reasons why advertisers would label their ads as political even if they are not: $(1)$ maybe Facebook's enforcement mechanisms labeled some of their ads as political, so for simplicity they label everything as political; $(2)$ advertisers think this will bring more attention to their page; or $(3)$ they understand better why their ads should be political.  While we cannot pinpoint the reason why these ads have disclaimers, the problem is that if we build automated detection mechanisms that take as input data from advertisers, the models will be affected by this noise, at least, and will be vulnerable to poisoning attacks, at worse. 
Hence, \textit{while enforcement mechanisms for flagging political ads that do not have the right disclaimer are essential,  the question is whether we should also have enforcement mechanisms for flagging ads that are non-political but have the political disclaimer.} 
% for different groups of ads (for plotting we consider unique advertisers). 


\begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.4]{plots/newvers_ads_categories_6ctg.pdf}
    \vspace{-3mm}
    \caption{NEW VERSION:Breakdown of ad message types for the different groups of ads with and without paid\_for\_by disclaimer.}
    \label{fig:ad_message_type_disclaimer}
       \vspace{-4mm}
\end{figure*}



\vspace{-1mm}
\paragraph{Analysis of ad messages with human annotators}
Figure~\ref{fig:ad_message_type_new} shows the breakdown of ad messages types for \opa. We can see ads with paid\_for\_by disclaimers cover a diverse set of ad types. To examine differences between what advertises label as political and what volunteers label as political Figure~\ref{fig:ad_message_type_disclaimer} shows the breakdown of ad types for \spa, \pa, and \pnpa with and without disclaimer separately.   
We can see from Figure~\ref{fig:ad_message_type_disclaimer} that \spa and \pa without disclaimers do contain a significant proportion of ads from highly political ad types such as 'political figure or political party' and 'elections' (59\% for \spa and 21\% for \pa). \textit{This adds to the evidence that some advertisers might willingly not declare their ads as political rather than being confused.}  

%\oana{discuss marginally political with label}

%\oana{problem with latex compilation, if I comment out the next paragraph it says fatal error}
%To better understand what ads are confusing advertisers each ad type we compute the fraction of ads that do not have a disclaimer in the \spa and \pa groups.  
To better understand what ads are confusing advertisers each ad type we compute the fraction of ads that do not have a disclaimer in the \spa and \pa groups. Ads about political values and governance(0.22), civil and social rights(0.42) and immigration(0.46) have the lowest fraction of ads with disclaimer, while ads about elections (0.72)({\color{red}0.70}), economy (0.71)({\color{red}0.60}), and political figures (0.58)({\color{red}0.55}) {\color{red}{health(0.72), election(0.7) and crime(0.66)}} have the highest fractions of ads with disclaimer.  \textit{This shows that advertisers are underreporting ads about social issues (that are considered political by volunteers) especially if they are about immigration or \sout{environment} {\color{red}{civil and social right}}.} {\color{red}{will re-check it}}



%\begin{table}[]
%    \centering
%    \footnotesize{
%    \begin{tabular}{||l|c|c|c|c||}
%    \hline
%        Ad type &\# ads & median \fr& median \fr&fr. ads\\
%          &  &  & workers& disclaimer\\
%        \hline
%        \hline
%       Election & 50 & 1&1 & 0.72\\
%        \hline
%        Political Figures & 149 & 1 &1& 0.58\\
%        \hline
%      Immigration & 22& 0.92 & 1&0.27\\
%        \hline
%     Economy & 14& 0.71 & 1&0.71\\
%        \hline
%        Health & 20& 0.86 &0.9& 0.45\\
%        \hline
%     Environmental politics & 42 & 0.8 &1& 0.38\\
%        \hline
%        Guns & 8 & 1&1 & 0.37\\
%        \hline
%        Civil and social rights &53 &  0.87 &1& 0.34\\
%        \hline
%        Crime & 7& 0.91 & 1 &0.43\\
%        \hline
%        Education & 11& 0.66& 0.6&0.45 \\
%        \hline
%        Political values & 9& 0.66 & 0.75&0.33\\
%        \hline
%        Security and foreign policy & 3& 0.62 & 1 & 1\\
%        \hline
%    \end{tabular}
%    }
%    \caption{Median \fr and fraction of ads with paid\_for\_by disclaimer for different ad type for \spa and \pa.}
%    \label{tab:pa-spa ads ctg}
%\end{table}




% and this fraction is only 8\% if we look at ads in the \pa group that are also in the \opa group. The numbers are much 34\% and 2\% in the \pnpa group. 


%However, in the \pnpa group, the numbers are different. For \pnpa ads that are not in \opa, 34\% of ads have an advertiser that no longer exist and only 2\% of ads that have the official political label in \pnpa category do not havhe de the valid advertiser. Teference numbers between \pnpa and \pa groups may be caused by the fact that \pnpa group has less percentage political ads than other groups. 

%\oana{add similar numbers fro \pa and \pnpa}

%number of SP ads with label = 25387     number of SP ads without label = 11935 
%
%number of SP ads that come from an advertiser without category  = 10073
%
%number of SP ads without label that come from an advertiser without category = 7890 -- 2183
%
%in terms of unique advertisers: SP ads = 5356            number of SP ads without label = 1542                  number of SP ads without extracted categories= 1739                                                       number of SP ads without categories and without label = 1049

%We wanted to understand the difference between pages' categories from different types of political ads.

 %After that, we found the most popular categories for strong political, political and probably not political data.
 



%\update{Why labels from volunteers and workers differ. Maybe volunteers are influenced by the paid\_for\_by label -- ads with paid\_for\_by label get larger fractions of political votes. Volunteers might be better at recognizing political ads because ads were directly targeted at them. In our case Charlie Kirk is a politician, but the workers did not recognized this, they said the ad is about education}.  









==> labels_volunteers.tex <==
%!TEX root = paper.tex

\subsection{Analyzing ad labels from volunteers}
\label{sec:labels volunteers}

The ProPublica volunteers were given no instructions for what ads they should consider as political and users were left to decide based on their subjective beliefs and their personal background knowledge.  This provides us with a perspective on what ads people intrinsically consider as political and that can help craft better definitions and instructions for what is a political  ad. 

To understand what are the ads on which people agree and what are the ads on which people disagree we look at \textbf{consensus} between volunteers.  We consider consensus is a proxy for how complex the task of labeling political ads is.  Figure~\ref{fig:fr_votes_new} plots the distribution of the number of political votes divided by the number of all votes for each ad in the ProPublica dataset. We note this fraction as \fr.  A fraction \fr$=1$ means everyone agrees that the ad is political while a fraction \fr$=0$  means that everyone agrees that the ad is non-political. %
We split the ads in four disjoint \textit{ad groups} based on the volunteer votes:  

\vspace{-1mm}
\begin{itemize}
\item \textbf{\spa}:  where $\textit{fr}=1$
\item \textbf{\pa}: where $0.5\leq \textit{fr} <1$ 
\item \textbf{\pnpa}: where $0< \textit{fr} <0.5$ 
\item \textbf{\npa}:  where $\textit{fr}=0$
\end{itemize}
%\vspace{-1mm}

Table~\ref{tab:overlap} presents the number of ads in each group. There are 26k \spa, 19.7k \pa, 7.6k \pnpa and 1.3k \npa. Hence, for more than 50\% of the ads there is at least one volunteer that disagrees with the others, which shows that \textit{deciding if an ad is political is confusing in close to half of the cases.}  To understand why the task is complex, we check if there are any evident patterns between ads on which people agree and ads on which people do not agree.  We look next at who are the advertisers who send the ads and what issue the ad messages are addressing in the different ad groups. 


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.4]{plots/ECDF_new.pdf}
    \caption{ECDF of the fraction of political votes divided by all votes for the ads in the ProPublica dataset.}
    \label{fig:fr_votes_new}
\end{figure}

 \begin{table}[t]
 \small{
 \begin{tabular}{|l c c c|} 
 \hline
   & All & Official pol. & Official non-pol.  \\ %[0.35ex] 
\hline\hline
\spa & 26k &96\%& 4\%\\
  \hline
\pa & 19.7k& 93\%&7\%\\
  \hline
\pnpa & 7.6k & 74\% & 26\%\\
 \hline
\npa & 1.3k & 100\% & NA$\dagger$\\
\hline
\end{tabular}
}
\caption{\label{tab:overlap} Number of ads in different ad groups (based on volunteer votes) and overlap with ads labeled as political by advertisers. $\dagger$ ProPublica was not able to give us access to ads that did not have at least one political vote or that were not labeled as official political ads.} 
\vspace{-9mm}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.4]{plots/ads_merg_ct11_new_1.pdf}
    \vspace{-3mm}
    \caption{Breakdown of advertisers categories for ads in different groups of ads.}
    \label{fig:all_categories_new}
    \vspace{-5mm}
\end{figure*}

\vspace{-1mm}
\paragraph{Analysis of advertiser categories}
Advertisers need to create a Facebook Page and select from a pre-defined list a category for their page such as ``Software Company'' or ``Political Party''~\cite{adv_ctg_instr}.  We use the advertiser's ids available in the dataset to collect their category using the Facebook Graph API.  %The main category appears below the page name. To get advertiser's categories(any other data from Facebook) using a python code you need to register as a developer on Facebook and then have an access token. After that, we used Facebook library for python to collect categories from different advertisers. 
Some pages no longer exists, we were able to extract categories for 6476 ProPublica advertisers (82\%).
Figure~\ref{fig:all_categories_new} plots the breakdown of the advertisers categories for \spa, \pa and \pnpa. There are 9342 unique advertiser categories in the ProPublica dataset,
Figure~\ref{fig:all_categories} only shows categories that are shared by more than 1\% of advertisers. We also group together similar advertiser categories (see Appendix, Table~\ref{tab:cls categories rules} for grouping details). 

Figure~\ref{fig:all_categories_new} shows that most \spa come from political actors (57\%), some from NGOs (15\%), but we also see some ads from communities (4\%), advocacy groups(4\%), news media (1\%) and businesses (1\%).

In the \pa group, a smaller fraction of ads come from political actors (23\%) and advocacy groups (6\%), much more from NGOs (37\%) and we also see more ads from news organizations (4\%), communities (6\%), and businesses (2\%). 

In the \pnpa group, 1\% of the ads come from political actors, the majority (54\%) come from NGOs, some ads come from news medias (5\%) and businesses (4\%), and we also see many ads coming from charity organizations (9\%). \textit{These results show that a vast range of advertisers are pushing political ads online and that volunteers label ads as political from a diverse set of advertisers.  
Hence, definitions of political ads such as the one from Twitter that focuses only on political actors are too narrow.}  Similarly, Facebook is explicitly exempting news organizations from labeling their ads as political even if they talk about political issues~\cite{facebook-political-ads}, however, volunteers do consider these ads as political. 







%\begin{table}[]
%\footnotesize{
%    \centering
%    \begin{tabular}{|l|c|}
%    \hline 
%        Category & Median \fr \\
%    \hline
%    \hline
%       Political actors  &  1\\
%       \hline
%       Advocacy group & 0.8\\
%       \hline
%       Community & 0.96\\
%       \hline
%       Charity & 0.28\\
%       \hline
%       Cause & 0.8\\
%       \hline
%       NGOs &0.7\\
%       \hline
%       Public Figure & 1\\
%       \hline
%       News media & 0.66\\
%    %   \hline 
%     %  Medical and health & 0.66\\
%       \hline
%       Education & 0.68 \\
%       \hline
%       Business & 0.66\\ 
%       \hline
%    \end{tabular}
%    \caption{Median \fr for different advertiser categories.}
%    \label{tab:med_adv}
%    }
%\end{table}

To see if ads from certain categories of advertisers are more confusing, for each advertiser category we group all corresponding ads and we compute the median \fr of the group:  
\vspace{-1mm}
\begin{trivlist}
\item \hspace{2mm}  \textit{Political actors (1);  Advocacy group (0.8); Community (0.96); Charity (0.28); Cause (0.8);  NGOs (0.7); Public Figure (1); News media (0.67); Education (0.68); and Business (0.67).}
    \end{trivlist}
    \vspace{-1mm}
    

%We see that ads coming from clear political actors achieve a median \fr of 1, ads from NGOs, news organizations and businesses have a median \fr of 0.7, 0.66 and 0.66 respectively, and charities have a median \fr of only 0.28. 
Ads with a median close to 0.5 are the most confusing (half of volunteers label them as political and half as non-political),  hence, ads from NGOs, news medias, education and business are the most confusing.  These ads are more confusing,  either because they come from advertisers that are not classical political actors, either because the message of the ads is not clearly political.  While a conjoint analysis that tests the same ad message with different advertisers is needed for getting definite proof of how the advertiser category influences the decision, a close look at ads in these categories shows that even if we ignore the advertiser, some of the ads are clearly political while other as more confusing (see Table~\ref{tab:exmp_adv_ctg_diff} in Appendix). The ads address a wide range of topics (e.g., abortion, wildlife, violence, hunger), they call for various actions (e.g., sign petitions, vote, surveys, donations) and try to provoke various sentiments (e.g., pride, anger, fear). 
\textit{To reduce the number of ads that are confusing, platforms and policy makers should clarify how much consideration should be given to the advertiser when labeling ads as political or if the advertiser should be ignored altogether.} %Since, irrespective of the advertiser, some ads are confusing because of their message, we look next at ad messages. 


%\textit{These results show that there are differences between the advertiser's categories in ads on which people agree and ads on which they do not agree and that some categories of advertisers are more confusing than others. } 


%To see whether ads from certain categories of advertisers are more confusing than other ads, 




%


%The reasons why people disagree on what is a political ad are diverse.
%To understand whether the advertiser plays a role, 

\paragraph{Analysis of ad messages with human annotators} 
%To analyze the ad message we took a random sample of 200 ads from the three categories \spa, \pa and \pnpa and set up a Prolific~\cite{prolific} experiment where we asked workers about what is the ad message. 
To further study what ads volunteers find  confusing we gathered data about the issues discussed in the ad messages. We took a random sample of 100 ads with paid\_for\_by disclaimer and 100 ads without paid\_for\_by disclaimer from the \spa, \pa \pnpa and 200 \npa and set up a survey on Qualtrics~\cite{qlt} where for each ad we ask people questions about the message of the ad. We picked both ads with and without disclaimer because volunteers might have been influenced by this visible tag when labeling ads as political. We hired workers through Prolific~\cite{prolific} and we redirected them to fill out the survey on Qualtrics. Each worker had to label 20 random ads from the pool of 800 ads and each ad was labeled by three workers. 

%\oana{actually it is not a random sample of 200 ads, is  100 without disclaimer and 100 with disclaimer no?} \oana{can you send me a figure like figure 3 but where you have 6 bars corresponding to the different groups and with/without disclaimer}

For each ad the workers had to decide (level 1) if the ad is \textit{political} or \textit{non-political}  (see Figure~\ref{fig:sr_def}). For political ads (level 2) whether it is from or about a \textit{political figure or political party}, whether it is about \textit{elections or voting} or whether it is about a \textit{social issue}. For social issue ads (level 3), workers had to choose which type of social issue from the following list : \textit{civil and social rights}, \textit{crime}, \textit{economy}, \textit{education}, \textit{environmental politics}, \textit{guns}, \textit{health}, \textit{immigration}, \textit{political values and governance}, \textit{security and foreign policy}. We considered these types of social issues because they are the social issues that appear in the Facebook definition of political ads~\cite{soc_issue}.

Figure~\ref{fig:ad_message_type_new} shows the \textit{type} of ad messages according to Prolific workers for different ad groups.  Workers were allowed to choose multiple social issues for each ad. 
%For 255 ads the three workers agreed on the ad type, for 568 two out of three workers agreed on the ad type, and for 32 ads each worker chose a different ad type. 
For each ad, we pick the ad type choose by the majority of workers or mark it as disagreement if no two workers choose the same ad type. 

%ads_categories_dis.pdf
\begin{figure*}
    \centering
    \includegraphics[height=0.15\textheight]{plots/newvers_ads_categories_4ctg.pdf}
    \vspace{-4mm}
    \caption{NEW VERSION: Types of ad message in different groups of ads.}
    \label{fig:ad_message_type_new}
    \vspace{-4mm}
\end{figure*}


Figure~\ref{fig:ad_message_type_new} shows that all groups of ads contain most of the ad types we consider. We see higher fractions of ads from or about political figure or political party and ads about election in the \spa (66\%) and higher fractions of social issues ads in the \pa (35\%) and \pnpa (36\%). This tells us that \textit{a large proportion of the ads volunteers label as political are about social issues and not only about political actors. Social issue ads are only considered as political by Facebook and TikTok, and not by Google and Twitter. Hence, from ordinary people's perspective, it is important to consider these ads as political as well. In addition, the results tell us that social issues ads are more confusing.}
%


 
To understand whether some ad types are considered more or less political by volunteers, for each ad type, Table~\ref{tab:ads social iss} presents the median \fr as well as the fraction of ads with the paid\_for\_by disclaimer.  We see that some social issues get more political votes than others: ads about immigration and guns have a high median \fr (0.89 and 1) while ads about environmental politics and security and foreign policy have a low median \fr (0.39 and 0.3). This bias does not seem to be influenced by paid\_for\_by  disclaimers as they do not appear more often on ads about social issues with high \fr than social issues with low \fr.  Hence, there are two explanations for these variations, either that some issues are considered more political than others (maybe volunteers are getting biased by the information they get exposed to), either that the precise content of the ad is more politicized for some issues. \textit{The question for policymakers 
is who should decide what social issues should be considered as political, should all social issues be considered equally political and what would be a good granularity for defining a social issue. For example,  ads about guns are quite specific but ads about civil and social rights contain ads about several important issues such as abortion, LGBT or prisoners that can be more or less politicized.}  It is also worth thinking what happens if a new social issue arrises, or an old issue is becoming more politicized. We need ad moderation systems that are able to adapt in time and across locations and we need clear policy recommendations to arrive there. 

%To see whether ads, talking about the same social issue, with higher \fr have more politicized content than ads with low \fr.  
Finally, the question still standing is why for a particular social issue, some ads have higher \fr than others.
Tables~\ref{tab:exmp_pnpa_civ}-\ref{tab:exmp_pnpa_env} (in Appendix) show examples of civil and social rights  ads and environmental politics ads for different ad groups. For environmental politics ads we see that ads in the \spa often talk about legislation, congress or politicians, \pa ads have more advocacy messages and \pnpa ads have advocacy messages as well but about wildlife. Contrary, for civil and social rights the distinction between ads in different groups is not so clear.   
\textit{The questions that needs to be discussed is whether ads that address the same social issue but that are more politicized should be treated differently than ads that have a more informative message. Should we treat as political only ads that discuss a direct impact on legislation or should we also consider as political ads with an indirect impact? In all, these results show again the complexity of labeling political ads.} 


% Even if there might be ways to train workers and volunteers to reduce confusion through more precise policies, there are still ads where the confusion cannot easily be alleviated. 

\vspace{-1mm}
\paragraph{Volunteers vs. workers}
Figure~\ref{fig:ad_message_type_new} shows some disagreement between workers and volunteers on 4\% of \spa and 28\% of \pa that are marked by at least two of three workers as non-political. Since there is no available expert ground truth, we cannot say whether labels from volunteers or labels from workers are better, but we can try to investigate reasons behind disagreement. Workers were also asked to choose a topic for the ad message even if they labeled the ad as non-political (the topics were selected from the IAB list~\cite{adv_ctg}). The topics that were mentioned the most by workers for these ads are Society, Health \& Fitness, Education and Science. \textit{This raises the question of where should we draw the line between ads about social issue and ads about Society; or ads about social right and Health \& Fitness?}   Another possible reason is that workers and volunteers have different background knowledge that influences their decision and volunteers might be better at identifying political ads than workers as the ads are directly targeted to them.


We see anecdotal proof for this for an ad with $\textit{fr}=1$ but labeled as non-political by three workers: ``Hello everyone- please click this link to read my legislative wrap up newsletter. Have a great evening. Kirsten Enge''.  Kirsten Engel was a member of Arizona House of Representatives. {\color{red}{we do not have this ad in the dataset anymore}}


We see a proof for this for an ad with $\textit{fr}=0.83$ but labeled as non-political workers:
{\color{red}{''We outraised Susan Collins last quarter without taking a dime of corporate PAC money. Help us keep that up by making a 5\$ grassroots contribution now.'' by Sara Gideon. Susan Collins is a United States senator and advertiser Sara Gideon is a former ME State Representative}}

It is possible that workers did not have the appropriate background knowledge to know she is a political actor {\color{red}{they are  political actors}}. Hence, \textit{background knowledge is an important component to consider when gathering political ad labels on crowdsourcing platforms.} \textit{Workers might also be more superficial when deciding if an ad is political or not. Hence, it might be worth working with experts to create a gold standard collection for political ads especially social issue ads.} 








%\oana{@vera: can you give me more examples of these ads that are marked as non political by workers?}
%\vera{Americans for Prosperity is excited to open up a new field office in Fargo! Join us on Tuesday, September 25 from 6-8 PM to network, enjoy great food and drinks, and learn how to join our fight for freedom. by Americans for Prosperity - North Dakota. $fr_v$ = 1, $fr_w$ = 0.33}
%\vera{Hundreds of Oregonians have spoken up for fair drug pricing. We can't stop now. by Oregonians for Affordable Drug Prices Now,$fr_v$ = 1, $fr_w$ = 0.33}
%\vera{We need your help! We’re ready to print more yard signs to put up all across FL-15, but we need to raise another \$5,850 to make our next order. Will you chip in \$5 (equal to 2 signs) so we can blanket the district with our campaign signs? by Kristen Carlson for Congress, $fr_v$ = 1, $fr_w$ = 0.33} \oana{what are the topics chose by these workers for the ads?}


Figure~\ref{fig:ad_message_type_new} shows that 4\% of the \pnpa do contain highly political ads such as  political figure or political party ads. Table~\ref{tab:exmp_pnp_ctg_elect} (in Appendix) shows a few examples of these ads. %We can see that, for example, volunteers did not considered  ads about senator Jeff Flake and Ruth Bader Ginsburg as political, and workers considered ads from Melinda Gates as political. \oana{I am really confused why they were not labeled as political by volunteers}

We also see that a considerable number of \pnpa are about social issues (according to workers). For example, 9\% of ads are about civil and social rights and 8\% are about environmental politics.  One possible reason for the disagreement is that the instrumentation of our ad labeling process on Prolific influenced workers (we asked them to label ads as political according to the Facebook definition, and we made them choose what social issue the ad is addressing) which made workers to identify better ads about social issues as political.  Section~\ref{sec:prolific} explores more in depth how different ad labeling instrumentations influence what workers label as political.  
\textit{These results also show that \pnpa should not be ignored because they might contain political ads where only few people have the right background knowledge to detect them.} 



%\oana{takeaway?} 
%\update{Finally, there are also 56\% of \pnpa that are consider by workers as non political. One explanation is that there is one volunteer that mistakenly labeled these ads as political. \vera{The median number of votes is 1 for workers, the same for volunteers}





%\vera{moreover, most of them were labeled as political or strong political in survey with definition.  The median fraction of political votes in survey with definition is 0.6. Many ads about environmental politics seems to be political as well. However, the median fraction of political votes in survey with definition is 0.33. SO definition helped people to understand that ads about civil and social right are political, but  environmental problems do not considered as social issues for many people}



%Hence, the question is why are these ads voted by many volunteers as being non political and should they actually be considered as political?   \oana{can you take some examples from these two categories to understand why they were not labeled as political?} \oana{maybe some people are just not considering ads about social issues as political - which can be fixed though a better definition?}
 


 

%First thing we can observe from the figure is that ads in the different groups of ads do cover a wide range of social issues.  We see that 64\% of \spa,  36\% of \pa and 10\% of \pnpa are about political actors or election and, in reverse, only 35\% of \spa ads are about social issue, 59\% of \pa and 68\% of \pnpa.



%Some social issues are considered less political than others. We have less ads about environmental politics in the \spa group than in the \pnpa group. Not sure if in terms of numbers is higher since we look at fractions. What we could do is to check out of all the ads considered as enironmental politics, how many are in the different groups/ 

\begin{table}[]
    \centering
    \footnotesize{
    \begin{tabular}{|l|c|c|c|c|}
    \hline
        Social Issue &\# ads & median \fr& median \fr&fr. ads\\
          &  &  & workers& disclaimer\\
        \hline
        \hline
         Election & 53 & 1&1 & 0.72\\
        \hline
        Political Figures & 164 & 1 &1& 0.58\\
        \hline
        Immigration & 24& 0.89 & 1&0.29\\
        \hline
        Economy & 23& 0.67 & 0.5&0.61\\
        \hline
        Health & 35& 0.6 &0.5& 0.41\\
        \hline
        Environmental politics & 94 & 0.39 &0.66& 0.54\\
        \hline
        Guns & 9 & 1&1 & 0.44\\
        \hline
        Civil and social rights &90 &  0.66 &0.75& 0.43\\
        \hline
        Crime & 12& 0.69 & 0.66&0.41\\
        \hline
        Education & 14& 0.63& 0.41&0.57 \\
        \hline
        Political values & 14& 0.66 & 0.71&0.57\\
        \hline
        Security and foreign policy & 11& 0.3 & 0.66&0.54\\
        \hline
    \end{tabular}
    }
    \caption{Median \fr and fraction of ads with paid\_for\_by disclaimer for every ad type.}
    \label{tab:ads social iss}
    \vspace{-10mm}
\end{table}


%\noindent \textbf{Takeaway:} 
 %As expected, we see an over representation of ads from political actors and ads about elections in the \spa group and an over representation of issue ads in the \pa and \pnpa groups, however, there is a significant fraction of ads from political actors.
  






==> prolific.tex <==
%!TEX root = paper.tex

\section{Impact of task design on ad labeling}
\label{sec:prolific}
This section investigates what effect has the ad labeling process on what ads humans label as political. We focus on two questions:  
\vspace{-1mm}
\begin{trivlist}
\item $Q_1$: \textit{How does the definition of what is a political ad impact ad labeling? }
\item $Q_2$: \textit{How does social influence impact ad labeling?} 
\end{trivlist}
\vspace{-2mm}

\begin{figure}
  \centering
  \includegraphics[scale=0.25]{plots/survey_with_dif.png}
  \caption{Example of ad we asked workers to label.}
  \label{fig:sr_def}
  \vspace{-6mm}
\end{figure}

%\begin{figure}
%  \centering
%  \includegraphics[scale=0.3]{plots/why.png}
%  \caption{Survey with definition: question about political ads}
%  \label{fig:why}
%\end{figure}


\subsection{Experiment design}
To answer these questions, we set up three experiments on Prolific where we asked workers to label ads as political or not. \textcolor{red}{We have selected workers that are residing in the USA. We had this selection criterion because all the ads used in the experiments were targeted at people who lived or visited in the USA. We paid workers £7.80 per hour. The median amount of time that workers spent on the survey were between 3.5 to 9.1 minutes, depending on the experiment's type.}Each survey had an instructions page, followed by 20 pages that contained one ad to label (see Figure~\ref{fig:sr_def}):

\begin{trivlist}
\item \hspace{2mm} $Exp_1$: In the first experiment we did not provide any definition. The instruction page only contained the message: \textit{In this survey, you will be asked to decide whether an ad is \textbf{political} or \textbf{non-political}.}
\item \hspace{2mm} $Exp_2$: In the second experiment, we gave in the instruction page the definition of political ads from Facebook, and we ask workers to label ads accordingly. 
%To ensure workers have permanent access to the definition, 
We included a link to the definition on every page of the survey. Also, we asked workers to motivate their choice for each ad by selecting from the list of reasons (presented in Section~\ref{sec:labels volunteers}) that were extracted from the Facebook definition for political ads. To match the quantity of work, we also asked workers to choose from a list of topics (taken from the IAB categories~\cite{adv_ctg}) when they were labeling an ad as non-political. 
\item \hspace{2mm} $Exp_3$: In the third experiment, we did not provide a definition, but, for each ad, we told workers what fraction of people labeled the ad as political previously (we used data from the $Exp_1$). 
\end{trivlist}

To create the surveys, we used Qualtrics~\cite{qlt}. To test the ad labeling process's influence on a wide range of ads, we took a random sample of 200 ads from \spa, 200 ads from \pa (100 with paid\_for\_by disclaimer, and 100 without a disclaimer) and 200 ads from \pnpa.  
Besides, we took 200 random ads without disclaimer from \AdAnalyst USA users. Note that we do not show whether the ad has a disclaimer or not in our surveys. We use the same ads in the tree experiments. For every ad in every experiment, we collected three labels.  Every participant was given a random sample of 20 ads to label from the 800. Workers were only able to participate in one experiment.

\subsection{Analysis of labels}



%Figure~\ref{fig:dist_plots_fr} plots distributions of the fraction of political votes for different %different groups of ads.
 
%

%Figure~\ref{XX} plots the CDF of \fr (the number of political votes divided by a number of all votes) obtained from the three experiments as well as the \fr of volunteers. We can see that \update{....} \oana{come back after plot is there}. \update{The number of political votes was increased after we defined political ads to the volunteers. All ads that have a fraction of political votes equal to 1 in the survey with the definition and a fraction of political votes less than 0.5 in the survey without a definition were labeled as ads about social issues. } \oana{i do not understand? we do not have ads about political actors?} 

To check if the impact on votes of our three experimental designs is statistically significant, we test the following two null hypotheses: 
\begin{trivlist}
\item $NH_1$: The definition of political ads does not impact labeling.
\item $NH_2$: Social influence does not impact labeling.
\end{trivlist}

To test the two hypothesis we check whether the distributions of the fraction of political votes for $Exp_1$ and $Exp_2$ are identical ($NH_1$) and if the distributions for $Exp_1$ and $Exp_3$ are identical ($NH_2$). 
To choose a proper statistical significance test, we use the Kolmogorov-Smirnov test to check whether votes from the three experiments are normally distributed or not. The distributions are not normal. Hence, we use the Mann-Whitney U test, which is a non-parametric test to compare two independent distributions as our statistical significance test. The null hypothesis (the distributions are identical) is rejected if $p_{value}$ is less than 0.05. The results show that we cannot reject $NH_1$ because it has $p_{value}=0.059$ and we cannot reject $NH_2$ because it has a $p_{value}=0.39$. 

We further investigate whether there is a statistically significant impact on specific groups of ads: \spa, \pa, \pnpa, and non-political ads.  
We use the Wilcoxon T-test to check, inside each experiment, if votes on \spa, \pa, \pnpa, and non-political ads come from the same distribution or not. We compare the four samples of data with each other. The results show that the distributions samples are different from each other, so it is good to analyze them separately. We proved that samples of distributions are not normal distribution by using the Kolmogorov-Smirnov test. 

\begin{table}[t]
  \small{
  \begin{tabular}{|l|c|c|}
  \hline
   	    & $NH_1$ & $NH_2$ \\
   %  & ($Exp_1$: no def. & ($Exp_1$: no def. \\
   %  & vs $Exp_2$: def)& vs $Exp_3$: fraction)\\
  \hline
   \hline
  \spa & 0.6 & 0.07 \\

  \hline
      \pa & \textbf{0.001} &  0.06 \\
  \hline
      \pnpa& \textbf{0.01} & \textbf {0.009} \\
    \hline
      \npa & 0.06 & 0.5\\
  \hline
  \end{tabular}

  \caption{$p_{value}$ from the Mann-Whitney U test for different groups of ads to verify $NH_1$ ($Exp_1$: no def. vs $Exp_2$: def) and $NH_2$ ($Exp_1$: no def. vs $Exp_3$: fraction).}
  \label{tab: MWU}
}
\vspace{-8mm}
\end{table}



Table~\ref{tab: MWU} shows the $p_{value}$ for the different groups of political ads between different experiments. The null hypothesis is rejected only for \pnpa and $NH_1$. This shows that even if the definition for political ads did not significantly impact \spa and \pa, it did have a strong impact on \pnpa. This is good because these are the ads that are the most confusing and problematic. 
Contrary, $NH_2$ is not rejected for any group of ads, hence providing information about how other people labeled ads did not affect votes. 

\begin{figure*}[t]
 % \begin{minipage}{0.16\textwidth}
  % \centering
  \subfloat[\spa]{\includegraphics[width=0.25\textwidth]{plots/dist_plots_sp.pdf}}
  % \end{minipage}\hfill
 % \begin{minipage}{0.15\textwidth}
  % \centering
  \subfloat[\pa]{\includegraphics[width=0.25\textwidth]{plots/dist_plots_p.pdf}}
 % \end{minipage}
  % \begin{minipage}{0.15\textwidth}
  % \centering
   \subfloat[\pnpa]{\includegraphics[width=0.25\textwidth]{plots/dist_plots_pnp.pdf}}
 % \end{minipage}
   \vspace{-3mm}
   \caption{Distribution of the fraction of political votes for different groups of ads and different experiments.}
   \label{fig:dist_plots_fr}
   \vspace{-5mm}
\end{figure*}

%\oana{here is a paragraph that is giving me a fatal error}
Figure~\ref{fig:dist_plots_fr} plots distributions of the fraction of political votes for different groups of ads. The number of political votes increase in all presented groups of ads in the $Exp_2$, and this difference the highest in the case of \pnpa. Hence, providing the Facebook definition determined workers to see more political content in ads; however, the agreement does not seem to increase. This means there is room for improvement on both political ad definition and the ad labeling process's instrumentation. 

%Around 20\% of \pnpa have fraction of political votes more than 0.5 in $Exp_2$ and less than 0.5 in $Exp_1$ and in $Exp_3$. We can conclude that after we defined political ads to the workers, they started seeing more political content in the ads. However, $Exp_2$ still has a big fraction of \pnpa.
%
%


\paragraph{Discussion}
From an ad moderation perspective, a consensus is desirable because the decision of what is a political ad is clear and is straightforward to exploit the labels to build automated ML algorithms to detect political ads. However, consensus alone is not enough; for example, if we ask French people to label US political ads, they might only label ads from Donald Trump but nothing else because they are not familiar with US politics. French volunteers will have a perfect consensus, but they will miss many interesting political ads. Hence, a second critical dimension is the \textbf{diversity} of ads labeled. Ideally, we want to throw a large nest that can capture explicit political ads from presidential candidates. However, we would also want to capture ads coming from local candidates and new social issues that arise in particular groups of people that are not well known nationally. Hence, ad labeling guidelines should attempt to increase consensus but not at the detriment of diversity. 

